Parallel Coordinate Descent Newton Method for Efficient $\ell_1$-Regularized Minimization

The recent years have witnessed advances in parallel algorithms for large scale optimization problems. Notwithstanding demonstrated success, existing algorithms that parallelize over features are usually limited by divergence issues under high parallelism or require data preprocessing to alleviate these problems. In this work, we propose a Parallel Coordinate Descent Newton algorithm using multidimensional approximate Newton steps (PCDN), where the off-diagonal elements of the Hessian are set to zero to enable parallelization. It randomly partitions the feature set into $b$ bundles/subsets with size of $P$, and sequentially processes each bundle by first computing the descent directions for each feature in parallel and then conducting $P$-dimensional line search to obtain the step size. We show that: (1) PCDN is guaranteed to converge globally despite increasing parallelism; (2) PCDN converges to the specified accuracy $\epsilon$ within the limited iteration number of $T_\epsilon$, and $T_\epsilon$ decreases with increasing parallelism (bundle size $P$). Using the implementation technique of maintaining intermediate quantities, we minimize the data transfer and synchronization cost of the $P$-dimensional line search. For concreteness, the proposed PCDN algorithm is applied to $\ell_1$-regularized logistic regression and $\ell_2$-loss SVM. Experimental evaluations on six benchmark datasets show that the proposed PCDN algorithm exploits parallelism well and outperforms the state-of-the-art methods in speed without losing accuracy.

==> defs_jmlr.tex <==
\usepackage{jmlr2e_cus}
\usepackage[usenames]{xcolor}
%\usepackage[usenames]{color}
\usepackage[bookmarksnumbered=true]{hyperref}
\usepackage{url}
\definecolor{cite_color}{RGB}{0, 51, 153}
%\definecolor{link_color}{RGB}{0, 51,0}
%\definecolor{link_color}{RGB}{0,102,102}%  green-style
\definecolor{link_color}{RGB}{153, 0,0}  %  red
\definecolor{url_color}{RGB}{153, 102,  0}
\definecolor{emp_color}{RGB}{0,0,255}
% {51, 102, 51}
\hypersetup{
 colorlinks,
 citecolor=cite_color,
 linkcolor=link_color,
 urlcolor=url_color}
 % graph
\graphicspath{{./figs/}}

 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{multirow}
\usepackage{booktabs}
%\usepackage{mathrsfs} 
\usepackage{wrapfig}
\usepackage{enumerate}
\usepackage{bm}
%\usepackage{bbm}
% to use \bm in section title 
\pdfstringdefDisableCommands{%
	\renewcommand*{\bm}[1]{#1}%
	% any other necessary redefinitions 
}
\usepackage{tabularx}
% citation 
\usepackage{natbib}
\bibpunct{(}{)}{;}{a}{,}{,}
%1 the opening bracket symbol, default = (
%2 the closing bracket symbol, default = )
%3 the punctuation between multiple citations, default = ;
%4 the letter `n’ for numerical style, or `s’ for numerical superscript style, any other letter for author-year, default = author-year;
%5 the punctuation that comes between the author names and the year
%6 the punctuation that comes between years or numbers when common author lists are suppressed (default = ,);
\bibliographystyle{icml2017}
%  abbrvnat  plainnat icml2017
\usepackage{mathtools}



% For algorithms, use algorithm2e
\usepackage[vlined, ruled, linesnumbered]{algorithm2e}
%set comment style
\newcommand\mycommfont[1]{\footnotesize\textit{
\hspace{-.3em}#1}}
\SetCommentSty{mycommfont}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

 \usepackage{cleveref} % should be put after other packages 
 %  using always captial letter
 \crefname{section}{Section}{Sections}
 \crefname{theorem}{Theorem}{Theorems}
 \crefname{lemma}{Lemma}{Lemmas}
 \crefname{equation}{Equation}{Equations}
 \crefname{proposition}{Proposition}{Propositions}
 \crefname{claim}{Claim}{Claims}
% \crefname{algorithm}{Algorithm}{Algorithms}
   \crefname{algorithm}{Alg.}{Algorithms}
 \crefname{figure}{Fig.}{Figures}
 \crefname{table}{Table}{Tables}
 \crefname{remark}{Remark}{Remarks}
 \crefname{definition}{Definition}{Definitions}
 
 %In the first argument of \crefname{}{}{} comes the type of reference (equation, figure, table, section, etc.). The second argument contains the word that is printed if only one reference is made and the third argument contains the plural form for multiple references.
%  \crefname{equation}{Equation}{Equations}
%  \crefname{proposition}{proposition}{propositions}
%  \crefname{claim}{claim}{claims}


\newcommand{\todo}[1]{\textcolor{red}{@todo:}#1}
\newcommand{\appendixtitle}[1]{
	\begin{center}
		\LARGE \bf #1
	\end{center}
}

\def\C{{\cal C}}
\def\S{{\cal S}}
\def\E{{\mathbb E}}
\def\X{{\cal X}}
\def\Y{{\cal Y}}
\def\H{{\cal H}}
\def\Z{{\mathbb Z}}
\def\L{{\cal L}}
\def\N{{\cal N}}

\def\cone{{\cal K}}

\def\A{{\mathscr A}}
\def\M{{\cal M}}
\def \I {{\cal{I}}}
\def\T {\mathbb{T}}
\def\opt{\ensuremath{\Omega^*}}


\def \c{\bm{c}}
\def \v{\bm{v}}
\def \w{\bm{w}}
\def \r{\bm{r}}
\def \b{\bm{b}}
\def \d{\bm{d}}
\def \a{\bm{a}}
\def \x{\bm{x}}
\def \y{\bm{y}}
\def \s{\bm{s}}
\def \e{\bm{e}}
\def \u{\bm{u}}



\def \BA{\mathbf{A}}
\def \BB{\mathbf{B}}
\def \BX{\mathbf{X}}
\def \BY{\mathbf{Y}}
\def \BI{\mathbf{I}}
\def \BC{\mathbf{C}}
\def \BD{\mathbf{D}}
\def \BE{\mathbf{E}}
\def \BH{\mathbf{H}}
\def \BL{\mathbf{L}}
\def \BM{\mathbf{M}}
\def \BG{\mathbf{G}}
\def \BP{\mathbf{P}}
\def \BQ{\mathbf{Q}}
\def \BS{\mathbf{S}}
\def \BU{\mathbf{U}}
\def \BV{\mathbf{V}}
\def \BW{\mathbf{W}}
\def \BZ{\mathbf{Z}}

\def \BLambda{\mathbf{\Lambda}}  % B or b, depend on the first letter of the symbol
\def \BSigma{\mathbf{\Sigma}}
\def \bsigma{\bm{\sigma}}
\def \btheta{\bm{\theta}}
\def \blambda{\bm{\lambda}}
\def \balpha{\bm\alpha}
\def \bphi{\bm{\phi}}


\def \P{{\cal{P}}}
\def \Q{{\cal{Q}}}
\def \W{{\cal{W}}}
\def \B{{\cal{B}}}
\def \R{{\mathbb{R}}}
%  the transpose
\def \trans{\top}
% trace
\newcommand{\tr}[1]{\text{tr}(#1)}
\newcommand{\pare}[1]{{(#1)}}  % parethese sth, with extra {} added, used in a
% math mode


\def \z{\bm{z}}
\def \h{\bm{h}}

\def \D{{\cal{D}}}
\def \V{{\cal{V}}}
\def \E{{\mathbb{E}}} %  expection

\newcommand{\ALG}{Alg. }
\newcommand{\SEC}{{\textsection}}
\newcommand{\EQ}{Eq. }
\newcommand{\FIG}{Fig. }
\newcommand{\MAXCUT}{{\textsc{MaxCut}}}
\newcommand{\LOVASZ}{Lov{\'a}sz }

\newcommand{\argmin}{{\arg\min}}
\newcommand{\diag}{{\text{diag}}}
\newcommand{\dom}[1]{{\texttt{dom}(#1)}}
\newcommand{\sign}[1]{{\text{sign}(#1)}}
\newcommand{\dep}{{\text{Dep}}} % dependency set of a set function
\newcommand{\var}{{\text{Var}}} %  variance
\newcommand{\argmax}{{\arg\max}}
\newcommand{\algname}[1]{{\textsc{#1}}}
\newcommand{\note}[1]{\textcolor{blue}{//}#1}
%\newcommand{\spt}[1]{{\texttt{supp}^+}(#1)}
\newcommand{\spt}[1]{{\texttt{supp}}(#1)}
\newcommand{\dtp}[2]{\langle #1, #2\rangle}% dot product
\newcommand{\de}[1]{\text{det}\left(#1\right)}% determinant of a square matrix
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\fracppartial}[2]{\frac{\partial^2 #1}{\partial #2}}


\newcommand{\lleq}{\preceq}
\newcommand{\ggeq}{\succeq}
\renewcommand{\ll}{\prec}
\renewcommand{\gg}{\succ}

\newcommand{\bas}{\bm{e}} % standard basis

%% Standard
\newcommand{\groundset}{\ensuremath{\mathcal{V}}}


% new theorem
%
%\newtheorem{example}{Example}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{axiom}{Axiom}[section]
%\newtheorem{claim}{Claim}[section]
\newtheorem{assumption}{Assumption}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
